E-MPC: Edge-assisted Model Predictive Control

Model predictive control (MPC) has become the de facto standard action space for local planning and learning-based control in many continuous robotic control tasks, including autonomous driving. MPC solves a long-horizon cost optimization as a series of short-horizon optimizations based on a global planner-supplied reference path. The primary challenge in MPC, however, is that the computational budget for re-planning has a hard limit, which frequently inhibits exact optimization. Modern edge networks provide low-latency communication and heterogeneous properties that can be especially beneficial in this situation. We propose a novel framework for edge-assisted MPC (E-MPC) for path planning that exploits the heterogeneity of edge networks in three important ways: 1) varying computational capacity, 2) localized sensor information, and 3) localized observation histories. Theoretical analysis and extensive simulations are undertaken to demonstrate quantitatively the benefits of E-MPC in various scenarios, including maps, channel dynamics, and availability and density of edge nodes. The results confirm that E-MPC has the potential to reduce costs by a greater percentage than standard MPC does.

==> 6-Discussion.tex <==
%   | (Aug 22, 2024)
% ==================================================================================================
%   6  Discussion
% ==================================================================================================
\section{Discussion} \label{sec:discussion}

% In the E-MPC framework, by leveraging edge computing to empower agents, we propose three different methods exploiting the characteristics of edge networks. Firstly, increased computational capacity at the edge allows for more sophisticated MPC calculations. Allocating greater computational capacity at critical locations translates to evaluating a wider range of potential movement options and predicting more trajectories, leading to a more optimized path ultimately. However, deploying edge nodes with higher and varying computational power can increase hardware costs and introduce complexity in managing resource allocation across the network.

In the E-MPC framework, by leveraging edge computing to empower agents, we propose three different methods exploiting the characteristics of edge networks. Firstly, increased computational capacity at the edge allows for more sophisticated MPC calculations. Allocating greater computational capacity at critical locations translates to evaluating a wider range of potential movement options and predicting more trajectories, leading to a more optimized path. However, deploying edge nodes with higher and varying computational power increases hardware costs and introduces complexity in managing resource allocation across the network.

% Secondly, E-MPC allows for the natural incorporation of localized sensing information at the edge to improve state estimates. This real-time data feeding into the MPC process produces a more accurate understanding of the agent's environment, enabling an enhanced cost function. Thus, the agent can successfully take a detour from unexpected high-cost regions through the support from the edge. Nevertheless, this approach necessitates security measures to ensure the integrity and confidentiality of the localized sensing data processed and stored at the edge. Additionally, maintaining consistency of this information across numerous edge nodes requires careful design.

Secondly, E-MPC allows for the natural incorporation of localized sensing information at the edge to improve state estimates. This real-time data feeding into the MPC process produces a more accurate understanding of the agent's environment, enabling an enhanced cost function. Thus, the agent can successfully take a detour from unexpected high-cost regions through the support from the edge. Nevertheless, this approach necessitates security measures to ensure the integrity and confidentiality of the localized sensing data processed and stored at the edge. In addition, maintaining the consistency of this information across numerous edge nodes requires careful design.

% Finally, E-MPC utilizes localized observation histories to form empirical distributions and then samples predicted trajectories from the cost-optimal motion-primitive library. By analyzing past movement data, edge nodes can prioritize sampling motion primitives in areas frequently traversed by the agent. This targeted sampling improves the efficiency of the process and has the potential to lead to better path planning. However, this benefit has limitations. It may not be suitable for highly dynamic environments where past observations might not be indicative of future conditions. Additionally, storing historical observation data on edge nodes can lead to storage constraints and security concerns.

Lastly, E-MPC utilizes localized observation histories to form empirical distributions and then samples predicted trajectories from the cost-optimal motion-primitive library. By analyzing past movement data, edge nodes can prioritize sampling motion primitives in areas frequently traversed by the agent. This targeted sampling improves the efficiency of the process and has the potential to lead to better path planning. However, this benefit has limitations. It may not be suitable for highly dynamic environments where past observations might not be indicative of future conditions. Additionally, storing historical observation data on edge nodes can lead to storage constraints and security concerns.

% To sum up, edge computing offers significant advantages for optimizing local path planning through MPC. By strategically utilizing increased computational capacity, localized sensing information, and localized observation histories, agents can achieve more efficient and effective movement. Nonetheless, it's crucial to consider the trade-offs associated with each benefit, such as hardware costs, data security, and storage limitations, when designing and implementing an edge-based solution.
